A Blueprint for Precise and Fault-Tolerant Analog Neural Networks

Analog computing has reemerged as a promising avenue for accelerating deep neural networks (DNNs) due to its potential to overcome the energy efficiency and scalability challenges posed by traditional digital architectures. However, achieving high precision and DNN accuracy using such technologies is challenging, as high-precision data converters are costly and impractical. In this paper, we address this challenge by using the residue number system (RNS). RNS allows composing high-precision operations from multiple low-precision operations, thereby eliminating the information loss caused by the limited precision of the data converters. Our study demonstrates that analog accelerators utilizing the RNS-based approach can achieve ${\geq}99\%$ of FP32 accuracy for state-of-the-art DNN inference using data converters with only $6$-bit precision whereas a conventional analog core requires more than $8$-bit precision to achieve the same accuracy in the same DNNs. The reduced precision requirements imply that using RNS can reduce the energy consumption of analog accelerators by several orders of magnitude while maintaining the same throughput and precision. Our study extends this approach to DNN training, where we can efficiently train DNNs using $7$-bit integer arithmetic while achieving accuracy comparable to FP32 precision. Lastly, we present a fault-tolerant dataflow using redundant RNS error-correcting codes to protect the computation against noise and errors inherent within an analog accelerator.

==> text/3-1-discussion-analog-rns-ops.tex <==
\subsection*{RNS Operations in the Analog Domain}

% \subsubsection{Analog GEMM}
The RNS-based method requires modular arithmetic in the analog domain. 
The GEMM operations, e.g., convolution and fully connected layers, in the RNS space, can be achieved by performing a regular analog GEMM operation followed by a modulo operation in the analog domain. 
Analog GEMM is well-explored in the literature and can be realized by using various analog technologies. 
There have been many research efforts on optical GEMM---as a set of MVMs or dot products---mainly implemented by using Mach-Zehnder interferometers (MZIs)~\cite{CoherentNanophotonic2017} or microring modulators (MRRs)~\cite{weight-bank-2017}. 
Some other works leveraged PCM cells~\cite{feldmann2021parallel}, RRAM arrays~\cite{yao2020fully, prime-2016, isaac, 1t1m-2016, tang-2017}, STT-RAM~\cite{8241447, 9097177}, etc., for similar analog implementations.
For an RNS-based design, these GEMM implementations can be used as is but should be followed by an analog modulo operation. 
While the nature of modulo operation aligns with the digital representation of information and digital arithmetic systems, it can be performed in the analog domain. 

One way of performing analog modulo is to use ring oscillators\cite{analog-modulo-2018}.
A ring oscillator consists of an odd number of inverters that are connected as a ring where one inverter's input is connected to another inverter's output so that the signal keeps constantly switching between 0 and 1.
In this ring of inverters, where each inverter has a propagation delay $t_\text{prop}>0$, there is always only one inverter that has the same input and output---either 1-1 or 0-0---at any given time as the signal propagates in the ring. 
The location of this inverter with the same input and output also propagates along with the signal every $t_\text{prop}$ time and rotates due to the ring structure.
This rotation creates a modular behavior in the ring when the location of this inverter is tracked.

Another way of performing modulo in the analog domain is to use optical phase shifters. 
A phase shifter can shift the phase of a signal with an amount that is proportional to the length of the shifter and the applied voltage. 
These properties can be adjusted to encode two values (e.g., input and weight) and a phase shift proportional to the multiplication of these two values can be achieved.
By using a set of cascaded phase shifters, we can perform a modular dot where each phase shifter is programmed using two operands. 
As the phase values rewind at every $2\pi$, this behaviour is effectively a modulo against $2\pi$.
By scaling one set of residues (inputs or weights) by $2\pi/m$, modulo against arbitrary $m$ can be obtained. 

In addition, using RNS requires forward and reverse conversion circuits in the digital domain to switch between the RNS and the conventional number system. 
The forward conversion is a single modulo operation in the digital domain. The reverse conversion can be done using the CRT, mixed-radix conversion, or look-up tables. 
Hardware costs of these circuits can be reduced by using special moduli sets~\cite{hiasat1998residue, gallaher1997digit}. 

==> text/3-2-discussion-pns.tex <==
\subsection*{Extending the RNS with Positional Number System}
Using RNS achieves up to $\log_2M$ bit output precision in an analog GEMM core.  
It is possible to extend this range for both inputs and outputs and perform arbitrary precision fixed-point arithmetic in an analog core by combining the RNS with the PNS. 
% The combination of RNS and PNS with $D$ digits can provide up to $D \log_2M$ bit precision. 
By combining RNS and PNS, an integer value $Z$ can be represented as $D$ separate digits ($z_d$) where $d \in \{0, 1, ..., D-1\}$ and $0\leq z_d<M$:
\begin{equation}
    Z =  \sum_{d=0}^{D-1}z_dM^d,
\end{equation}
and can provide up to $D \log_2M$ bit precision. 
In addition, fractional fixed-point numbers can be represented by grouping the digits into two as $D_I$ integer digits and $D_F$ fraction digits. Then, $Z$ can be represented as
%(z_{D_I-1}\ z_{D_I-2}\  ...\  x_{0} \cdot x_{-1}\  x_{-2}\  ...\ x_{-D_F})$ can be represented as:
\begin{equation}
\label{eq:pns-fraction}
\begin{split}
      Z =  \sum_{d=0}^{D_I-1}z_dM^d +  \sum_{d=0}^{D_F-1}z_dM^d.
\end{split}
\end{equation}
This is synonymous with dividing the value by $M^{D_F}$.

This hybrid scheme requires carry propagation from lower digits to higher digits, unlike the RNS-only scheme. 
For this purpose, we can use two sets of moduli (primary and secondary)---similar to the RRNS idea used for error detection earlier---where every operation (e.g., addition, multiplication, or dot product) is performed both for primary and secondary residues. 
After every operation, overflow is detected for each digit by performing a base extension from primary to secondary moduli and comparing the base-extended residues against the secondary residues. 
The detected overflow is carried over to the higher-order digits within the PNS in the primary representation. 

